Tensor-Train Point Cloud Compression and Efficient Approximate Nearest-Neighbor Search

Nearest-neighbor search in large vector databases is crucial for various machine learning applications. This paper introduces a novel method using tensor-train (TT) low-rank tensor decomposition to efficiently represent point clouds and enable fast approximate nearest-neighbor searches. We propose a probabilistic interpretation and utilize density estimation losses like Sliced Wasserstein to train TT decompositions, resulting in robust point cloud compression. We reveal an inherent hierarchical structure within TT point clouds, facilitating efficient approximate nearest-neighbor searches. In our paper, we provide detailed insights into the methodology and conduct comprehensive comparisons with existing methods. We demonstrate its effectiveness in various scenarios, including out-of-distribution (OOD) detection problems and approximate nearest-neighbor (ANN) search tasks.

==> text/limitations.tex <==
\section{Limitations}
    While TT Point Cloud demonstrates an exellent ability to represent point clouds, one notable limitation of this approach is its inability to establish a direct one-to-one correspondence between points from the original point cloud and points from the TT point cloud.
    This constraint restricts its applicability to situations where the primary focus is on the underlying distribution rather than the original point cloud itself.
    For instance, TT Point Cloud is highly suitable for solving out-of-distribution (OOD) detection problems based on feature databanks and cannot be employed directly for nearest-neighbor search tasks.
    Nevertheless, we have shown how TT Point Cloud can still be utilized effectively in such scenarios as a first-stage search index structure.

